Enough Hot Air: The Role of Immersion Cooling

Air cooling is the traditional solution to chill servers in data centers. However, the continuous increase in global data center energy consumption combined with the increase of the racks' power dissipation calls for the use of more efficient alternatives. Immersion cooling is one such alternative. In this paper, we quantitatively examine and compare air cooling and immersion cooling solutions. The examined characteristics include power usage efficiency (PUE), computing and power density, cost, and maintenance overheads. A direct comparison shows a reduction of about 50% in energy consumption and a reduction of about two-thirds of the occupied space, by using immersion cooling. In addition, the higher heat capacity of used liquids in immersion cooling compared to air allows for much higher rack power densities. Moreover, immersion cooling requires less capital and operational expenditures. However, challenging maintenance procedures together with the increased number of IT failures are the main downsides. By selecting immersion cooling, cloud providers must trade-off the decrease in energy and cost and the increase in power density with its higher maintenance and reliability concerns. Finally, we argue that retrofitting an air-cooled data center with immersion cooling will result in high costs and is generally not recommended.

==> sections/ConcludingRemarks.tex <==
\section{Concluding Remarks}
In this paper, we explored the advantages and disadvantages of air cooling and immersion cooling for data centers. We evaluated these methods by looking at the various references as well as quantitative analysis presented throughout the paper. 

At this moment, most of the data centers around the world are relying on the air for cooling of their IT equipment, however, some providers are searching for a better cooling method and immersion cooling is recognized as an appropriate replacement. Such as any other technology, immersion cooling has some advantages and challenges compared to air cooling and providers need to select the best solution based on their specific application. The key findings of our study are as follows;

\begin{itemize}
    \item Referring to the reported PUEs for different data centers as well as the presented quantitative analysis on computing efficiency in this paper, it is concluded that the immersion cooling method consumes less energy and has a higher computing efficiency. Our analysis shows that a typical immersion-cooled data center consumes almost 50\% less energy compared to its counterpart air-cooled data center.
    \item Immersion-cooled data centers allow for much more compact designs, more than three times the density of their air-cooled counterparts. In liquid immersion-cooled data centers, there is no trade-off between efficiency and density. Conversely, air-cooled data centers can only be either-or. Immersion-cooled data centers can fit into small rooms with no need for a highly specialized environment. 
    \item While research on immersion cooling is mostly targeting efficiency, the aspect of computing density should not be overlooked. The increase of computing power in a specific volume is even more important than the efficiency improvement. Looking at the resources, the most conservative measurements of immersion cooling are about double the density in kW/l on rack-level compared to the maximum possible in air-cooled data centers. Resources estimating 4kW/l illustrate what is potentially possible with IT equipment optimized for liquid immersion cooling. This high-density capability, makes immersion cooling a perfect solution for running high-performance workloads. In addition, it allows manufacturing the CPUs and GPUs with higher frequency and higher power consumption.  
    \item The capital expenditure for an air-cooled data center with a power density of 10 kW per rack is about 4\% higher compared to its immersion-cooled counterpart. In addition, a 9-20\% operational expenditures reduction is expected with immersion cooling. 
    \item Mian downside of immersion cooling is maintenance challenges and reliability concerns. This is a reasonable explanation for why even with big advantages in efficiency and density by choosing immersion cooling, not many companies have switched their cooling solution to immersion cooling yet. This could be because there was not much information about reliability and maintenance and also available resources reported the maintenance procedure challenging.
\end{itemize}

As in any other area, it is important to select a solution based on the application usage. In General, even with all the advantages of immersion cooling, retrofitting an air-cooled data center with liquid cooling does not seem reasonable. In addition, considering the reliability and maintenance challenges and uncertainties, most of the providers find immersion cooling over-fitting for usual power densities. However, immersion cooling seams to be the best solution for high power densities.   

==> sections/cost.tex <==
An important factor to consider when adopting immersive liquid cooling are the capital and operational expenditures. The capital expenditures include a sealed chassis for immersing the IT equipment, dielectric fluids, as well as pumps and tubing. Similar to air-cooled data centers, the operational expenditures include electricity, staff, network connection fees, as well as supporting and maintaining the IT equipment.

According to \cite{Bunger2020}, for air cooled data centers with a power density of 10 kilowatt per rack, the capital expenditures are \$7.02 per Watt. For a liquid cooled data center with a similar power density, the cost is reduced slightly to \$6.98 per Watt. Of course, the benefit of liquid cooling is that much higher power densities can be achieved. When assuming a power density of 40 kilowatt per rack, the expenditures are further reduced to \$6.02 per Watt. Furthermore, when it comes to the operational expenditures, a reduction between 9-20\% is expected with regards to the energy cost due to the lack of fans. This is in agreement with \cite{Neudorfer2016}, who state that a 5-10\% reduction of the IT energy consumption is expected due the avoidance of internal fans. The need for fans is also removed from the facility side, reducing the total energy costs between 15-25\%. Another point to consider is that the dielectric fluids present in the sealed chassis can be used indefinitely, assuming some form of filtration is present. % according to https://multimedia.3m.com/mws/media/1838765O/3m-fluids-for-data-center-immersion-cooling-faq.pdf

In \cite{Day2019}, an important fact is highlighted: when building a new data center and optimizing it for liquid cooling from the ground up, capital expenditure savings can be achieved over air-cooled data centers. On the other hand, retrofitting an air-cooled data center with liquid cooling can result higher costs. An important exception is retrofitting an air-cooled data center that is limited on floor space and power capacity. In this case, the increased power density allowed by liquid cooling, as well as a reduction in energy consumption, can address both the space and power limitations of the air-cooled data center. 

%[A] R. Bunger, W. Torell, V. Avelar, “Capital Cost Analysis is of Immersive Liquid-Cooled vs. Air-Cooled Large Data Centers”, Schneider Electric White Paper 282, 2020.
%[B] J. Neudorfer, M. Ellsworth, D. Kulkarni, H. Zien, “Liquid Cooling Technology Update”, The Green Grid White Paper 70, 2016
%[C] T. Day, P. Lin, R. Bunger, “Liquid Cooling Technologies for Data Centers and Edge Applications”, Schneider Electric White Paper 265, 2019

